Machine learning based surrogate modeling with SVD enabled training for nonlinear civil structures subject to dynamic loading

The computationally expensive estimation of engineering demand parameters (EDPs) via finite element (FE) models, while considering earthquake and parameter uncertainty limits the use of the Performance Based Earthquake Engineering framework. Attempts have been made to substitute FE models with surrogate models, however, most of these models are a function of building parameters only. This necessitates re-training for earthquakes not previously seen by the surrogate. In this paper, the authors propose a machine learning based surrogate model framework, which considers both these uncertainties in order to predict for unseen earthquakes. Accordingly,earthquakes are characterized by their projections on an orthonormal basis, computed using SVD of a representative ground motion suite. This enables one to generate large varieties of earthquakes by randomly sampling these weights and multiplying them with the basis. The weights along with the constitutive parameters serve as inputs to a machine learning model with EDPs as the desired output. Four competing machine learning models were tested and it was observed that a deep neural network (DNN) gave the most accurate prediction. The framework is validated by using it to successfully predict the peak response of one-story and three-story buildings represented using stick models, subjected to unseen far-field ground motions.

==> figures/main.tex <==
\input{Front Matter}
\linenumbers
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\section{Introduction}\label{section1}
\comnt{georgios, please read this paragraph and feel free to edit} The performance-based earthquake engineering (PBEE) framework, developed at \cite{Cornell:2000}, is a powerful tool that can express performance of civil infrastructures during future earthquakes in terms of many useful decision variables (DVs). This framework relies on four successive steps that include hazard analysis, finite element simulation, mapping EDPs to damage measures (DMs), and finally, decision-making by translating DMs to various DVs. Despite being an excellent framework for performance assessment,  its use is limited in complex civil infrastructures due to high computational costs, that arises from non-linear probabilistic FE simulation of the structure, considering uncertainties in future earthquakes that require incremental dynamic analysis  and constitutive material parameters \cite{Parida2020,ZAKERESTEGHAMATI2021112971}. To alleviate this computational burden, researchers often use surrogate models to compute EDPs.In its most common form, a surrogate model aims to derive a low computational cost mathematical function that directly maps the inputs to the finite element model to its output, by-passing the computationally expensive non-linear analysis.  Often, this mapping function is developed based on fundamental structural dynamic theory in conjunction with Newtonian mechanics. Such physics based approaches have found wide use in earthquake engineering practice due to underlying physical robustness and intuitiveness \cite{Guan_2021}. However, these methods often rely on many inherent simplistic assumptions, which can reduce the accuracy of response estimates.Contrast to physics-based approaches, data driven approaches develop the underlying mathematical mapping function based on training on a large set of input-output data.  Recently, machine learning models like logistic regression (LR),  decision trees (DT), random forest (RF), support vector regression (SVR), artificial neural networks among others are finding  traction in the civil engineering community as viable data-driven surrogate models tp predict EDPs for their ease of implementation and ability to capture high degree of non-linearity \cite{Padgett_ML_review}.  LR, RF and SVR based surrogate models have been used in \cite{ATAEI2015203} for fragility assessment of the deck unseating mode of failure for coastal bridges.  Mangalathu et al.\cite{Mang_RF} used RF to generate and update bridge specific fragility curves and ANN \cite{Mang_ANN} to derive multidimensional seismic fragility of single and two column bent, box-girder bridges.  Segura et al. \cite{Segura} used a polynomial response surface surrogate model to construct fragility surface  for efficient seismic assessment of gravity dams.  In Ref.\cite{Mang_boost} machine learning techniques with boosting algorithms is used for response prediction of reinforced concrete frame buildings.  In the aforementioned studies and many other similar works \cite{MOLLER2009432, kocamaz_binici_tuncay_2021,WU_2019, PEREZRAMIREZ2019603, AHMED2022103737, KIANI2019108},  it has been clearly demonstrated that that once the machine learning model is properly trained, it can replicate a non-linear finite element model output accurately.  It must be noted that a considerable computational effort is expended in the initial training of the machine models to replicate the non-linear behavior of the structure,  however, the value in these methods is drawn from the fact once trained subsequent estimation of non-linear prediction are computationally trivial.  Most studies in literature, however, train the data driven surrogate model for a particular suite of earthquakes.  changing the earthquake suite would necessitate retraining the surrogate model for a new set of earthquakes, which would lead to more computational expense.  A few studies like in Ref. \cite{Taflanidis} use krigging surrogate model in conjunction with stochastic ground motion models to predict non-linear structural response.  Uncertain parameters of the ground motion models and finite element models are used as inputs to the surrogate model to predict the structural response.  Even though this approach is an effective solution to the aforementioned \comnt{repeated training problem} but this framework is limited to only when the seismic risk assessment utilizes stochastic ground motion models which is rarely the case.  \comnt{Georgios and supratik, please help me here, this citation, why this limitation is bad}. Additionally, krigging is not a reliable method sinc.. \comnt{Prashant, lets write this part}. The authors believe that in order for the surrogate model to have any meaningful application, one needs to develop a method that uses characteristics from historical earthquake data to train the surrogate models, along with accounting for high degrees of non-linearity that may arise during an earthquake. 


This research paper aims to propose a machine learning based framework that would address the repeated training problem along with being highly accurate in capturing larger degrees of non-linearity.  In effect, this is akin to solving three simultaneous problems a) identifying an exhaustive set of input parameters that are a good representation of historic earthquake data, b) identifying a set of input parameters that capture sensitivity of finite element model to its parameters and c) identifying the best machine learning model that is not only able to capture the high degree of non-linearity but also high degree of variation in response that may arise due to variation in earthquake and material parameters.  To this end, this paper first discuses a systematic framework for  development of the surrogate model in Section \ref{section2}. Different challenges that might arise for training a surrogate model in the context of earthquake engineering are discussed along with proposing an ideal workflow needed for development of surrogate model is proposed. Next, in Section \ref{section3}, a singular value decomposition based earthquake characterization technique is put forward that aims to characterize earthquakes in a way meaningful for generating training data for the surrogate model.  This is followed by a brief discussion of various machine learning models relevant for the proposed framework in Section \ref{section4}.  In Section \ref{section5}, the framework is applied to train machine learning models to replicate non-linear response of a single story and three-story building finite element model to earthquake excitation.  The framework is validated using earthquakes and material parameters which have not been used in training. 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\section{Systematic Development of the Surrogate model}\label{section2}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
As mentioned earlier the research team proposed a machine learning based surrogate modeling framework that can be easily integrated into the PBEE framework for computationally inexpensive decision making. The objective of the machine learning model would be to predict the EDPs for a finite element (FE) model, for an earthquake and a set of constitutive parameter values. A systematic surrogate model framework to predict for the given earthquake and the model would as follows
\begin{itemize}
\item Generate numerous time-histories ``similar" to the given earthquake and material parameters ``similar'' to the actual model parameters of the dynamic system.
\item Simulate the FE model for these time histories and material parameters.
\item Train a ``suitable'' machine learning model with the results of the FEM model as output and the corresponding material parameters and time history features as input till a pre-selected error tolerance is achieved.
\item Prior to deployment, the surrogate model needs to be validated with unseen earthquakes and material parameters that have not not used in training. Only if it predicts EDPs with reasonable accuracy then the machine learning model can be deployed.  
\end{itemize}
This implies that any systematic development of a machine learning based surrogate model should include three stages a) selection of suitable features and generation of training data b)  selection of suitable machine learning model and c) validation of the model and deployment.  These stages in context of the current study are discussed in the following. 

\subsection{Selection of suitable features and generation of training data }\label{subsec1}
In order to train the model,one needs to create a training set of input variables that should include characteristics of earthquake time history and building model parameters which would affect the prediction of EDP. Once the set of input variables are decided, the finite element model is simulated for different realizations of the input variables and the corresponding EDPs are stored. The machine learning model is now trained using input-output data sets till satisfactory convergence is attained. Such a supervised learning method is quite common and has been carried out by \cite{MOLLER2009432, Mang_boost, ZAKERESTEGHAMATI2021112971}. When this supervised learning technique is extended to account for earthquake and building material uncertainty, two important problems need to be addressed. First, the input features chosen should be exhaustive for predicting EDPs with certain degree of accuracy and second, it should be possible to draw realizations of those input features and simulate the finite element model using them in order to obtain training output. Traditionally, earthquakes have been characterized using single valued parameters like peak frequency, corresponding Fourier amplitude, peak ground acceleration (PGA), peak ground velocity (PGV), pseudo-spectral acceleration, Arias intensity, spectral moment, among others. From a training point of view, such characterization parameters pose a problem, since it is impossible to generate earthquake time histories for different realizations of these parameters i.e.  no inverse relationship exists between these intensity measures and earthquake time histories. This implies that such parameters are not unique to an earthquake. Not only selection of features is important, but also the existence of an inverse relation so that enough training data can be generated is imperative. Therefore, instead of using traditional intensity measures of earthquake characterization the authors have proposed an alternative framework as illustrated in Section \ref{section3}.

\subsection{Selection of suitable machine learning model}\label{subsec2}
Machine learning models have been widely used in literature of earthquake engineering to tackle different problems, including surrogate modeling \cite{ATAEI2015203,MOLLER2009432, kocamaz_binici_tuncay_2021,WU_2019, PEREZRAMIREZ2019603, AHMED2022103737, KIANI2019108} . Depending on the available data,  objective and the complexity of the problem,  available computational expenditure and desired level of accuracy various machine learning models, like the simplistic multiple linear regression,  to the more complex artificial neural networks are available to choose from. Moreover,  even for a machine learning model of choice, one can would need to tune its hyperparameters that in turn affect their accuracy and efficiency. drastically\comnt{cite prashant paper} \cite{mangalthu}.  For example for a neural network, the number of neurons and layers can be adjsuted to affect its accuracy and efficiency \cite{Papadrakakis}. One can also think of the number of polynomial terms and their orders as hyperparmeters for a simple linear regression problem.  Selection of machine learning models and selection of hyper-parameters need to be systematically handled and have been discussed further in Section \ref{section4}.

\subsection{Validation of model and deployment}
\comnt{Prashant Sid}

\section{Framework for ground motion characterization}\label{section3}
Consider a set of $n$ earthquakes with $m$ times steps each. Following the theory of singular value decomposition (SVD) \cite{ }, one can represent the $n \times m$ matrix $A_{n \times m}$ of $n$ earthquakes as:
\begin{equation}\label{PCA1}
A_{n \times m}=U_{m \times n}^T S_{m \times q} V_{q \times m }
\end{equation}
where, $U_{n \times p}$ and $V_{q \times m }$ are orthonormal vectors and $S_{p \times q}$ is a diagonal matrix. $u_i$, columns of $U^T$ and $v_i$, columns of $V$, form bases for $n-dimensional$ and $m-dimensional$ column spaces respectively. Choosing $U^T$ as my $n$-dimensional basis, Equation \ref{PCA1} can be written as:
\begin{equation}\label{PCA2}
A_{n \times m}=U_{n \times p}^T \Sigma_{p \times m}
\end{equation}
where, $\Sigma$ is the matrix obtained by product of $S$ and $V$ matrices. Each column of $\Sigma$ consists of weights for the $u_i$s to produce the original earthquake suite $A$. For example, $i^{th}$ column of $A$, can be produced by multiplying the basis matrix $U^T$ with $i^{th}$ column of $\Sigma$. Therefore every earthquake can be characterized by a $p$-dimensional vector which can be fed to the machine learning model.  Now, to create a training set one can generate $p-dimensional$ random vectors an use it to produce corresponding time histories needed for training. Moreover, any new earthquake $P_{n \times 1}$ that the machine learning model would be used to predict EDPs, for can be projected onto the $U^T$ basis:
\begin{equation}
\sigma_{p \times 1} = U_{p \times n}P_{n \times 1}
\end{equation}
to obtain the $p$-dimensional weight vector $\sigma$ which is then fed to the machine-learning algorithm to make predictions.
\comnt{prashant and sid, need to add more to make it clearer to understand}

Please note that, the number of input variables increase with $p$. However, this can be taken are of by selecting a few components of the basis vector matrix $U^T$. This can be better understood by understanding the principal component (PC) interpretation of SVD.
\comnt{A flow shart should be added here illustrating the framework} 
 
\subsection{Principal component interpretation of SVD}
\comnt{prashant and sid}
when you write the equation, mention the number of principal components used as $l$.. something like
fdfdfddf
\begin{equation}\label{PCA3}
A_{n \times m}=U_{n \times l}^T \Sigma_{l \times m}
\end{equation}

 \begin{figure}[h!]
\begin{center}
\includegraphics[width=0.9\textwidth]{figures/pca}

\caption{PDFSs}
\label{pdfs}
\end{center}
\end{figure}


\subsection{Drawbacks/Limitations}
Please not that SVD is a linear transformation. There are other methods like Kernel PCA \comnt{prashant}, etc which project the data to a set of non-linear basis. These transformation and their impact on machine learning prediction would be a part of the research teams future endeavors. 

\section{Competing set of machine learning models}\label{section4}
\comnt{prashant and sid}
As mentioned earlier selection of a machine learning model,  and tuning its hyper-parameters is a complex problem affecting the surrogate models accuracy and efficiency. Therefore, a systematic approach needs to be carried out for selection of a suitable machine learning surrogate model.After going through extensive literature four algorithms were selected to be candidate surrogate models. A brief description of the models have been provided in the following.

\subsection{Decision trees(DT) and Random forest regression (RF)} Decision trees recursively partition the input space based on local regression models in the input space.  A greedy optimization algorithm with the objective of minimizing the loss between the prediction of the tree and the actual measurement is utilized to find the optimal partition of the input space. To overcome potential over-fitting with a single tree, RF creates a large number of trees with different branches and depths and averages the output as its prediction.  Such a method is called \textit{bagging} where the average of a number of models result in an unbiased model. Number of DTs in the RF model and the maximum depth of each DT are two important tuning parameters that affect efficiency and accuracy of the prediction. 

\subsection{Support vector regression(SVR)} SVR use non-linear kernel function to map data into high-dimensional feature space. In this feature space, it is expected that the data attains more ``favorable" features which is then captured by a simple linear regression.  SVR is robust to over-fitting. and also provides flexibility by kernel selection.  Tuning parameters are type of kernel function, regularization parameter and  the allowed error tolerance ($\epsilon$) for the linear regression in high dimensional feature space.     

\subsection{Deep neural networks (DNN)} A deep network typically consists of an input layer, an output layer and a stack of hidden layers connecting the input layer to the output layer.  The hidden layers project the inputs into spaces of different dimensions via various linear and non-linear projections and produce the model output.  One hidden layer feeds into another via a linear transformation and within a hidden layer, the output of the previous layer is undergone a non-parametric non-linear transformation. The process is repeated for all hidden layers up until the output layers.  This stage is called forward propagation. Weights of the linear transformations can be obtained by minimizing the mean square error, loss between the model predicted output and the actual data.  This is done by back propagating the loss gradient via chain rule.  In this study, the rectified linear unit (ReLU) is used as non-linear transformation within a hidden layer \cite{}. This is because ReLU activation functions are more efficient and are generally shown to be best for deep neural networks because of fewer vanishing gradients problems when it is back-propagated through the hidden layers \cite{}. \comnt{Prashant} as compared to other activation functions like sigmoid.  

For DT, RF,  and SVR a cross validation approach is used to find optimal set of hyperparameters that best predict the data. In the case of DNN the optimal values of number of neurons and layers were decided heuristically by running several different number of neurons and layer combinations as suggested in \cite{Papadrakakis}.  Of the tuned machine learning models the winner is selected on the basis of some performance metric

\section{Results and Discussion}\label{section5}

\subsection{1Dof and 3Dof FEM models}
To illustrate the proposed framework,  one-story and three-story buildings are considered,  which are modeled as spring-mass-damper system in OpenSEES \cite{opensees}.  Chopra \cite{chopra2000dynamics} indicates that in most cases,  the first mode,  or the first few modes of a multi-degree of freedom stick model of the structure can provide useful approximation of the total response of the building,  and therefore, considered here. The springs are assumed to be uniaxial bilinear steel material with kinematic hardening with no isotropic hardening, and are modeled using the Steel01 \cite{} material in OpenSEES.  Elastic material element with specified damping stiffness was used in parallel with the non-linear spring to capture the damping behavior of the material.   For the one-story building, only one set of parallel springs are used, while for the three story building, three set of parallel springs are used in series. The objective of the problem is to accurately predict the response of these FE models for an earthquake,  using machine learning  given a set of values for spring constitutive model parameters.%The yield strength of the spring are so selected such that the response of the FE models reach the nonlinear regime,  so that we have enough data to capture the nonlinearity in training the surrogate model.  


\subsection{Choice of initial suite of ground motion}
As discussed earlier, the ground motion selection is one of the most important factors in training and developing accurate surrogate models, as the suite needs to be a good representation of an unseen excitation.  In this study, a set of 22 pair of ground motions representing magnitudes of range 6.5-7.6 recorded on firm soil (rock or stiff, $V_s$ > 180 m/s) were selected from the \cite{} \comnt{FEMA P695} far-field suite. The list of the selected ground motions and their characteristics are presented in \ref{table1}\comnt{Table 1}. All these ground motions are recorded at sites located greater than or equal to 10 km from fault rupture (strike slip and reverse thrust), referred to as “Far-Field” motions. To ensure broad representation of different recorded earthquakes, this set contain far-field records selected from most large-magnitude events in the PEER NGA database \cite{} \comnt{PEER, 2006}. The inherent differences in event magnitude, distance to source, source type and site conditions of these ground motions considers the record-to-record variability that is essential to capture the ground motion uncertainties. More information on the record selection criteria can be found in \cite{} \comnt{FEMA P695}. Figure \ref{eq_suite} shows the acceleration time histories of one component from each pair of ground motion in the earthquake suite. 
\begin{figure}
\begin{center}
\includegraphics[valign=c,width=0.19\textwidth]{figures/eq_0} 
\includegraphics[valign=c,width=0.19\textwidth]{figures/eq_2} 
\includegraphics[valign=c,width=0.19\textwidth]{figures/eq_4}
\includegraphics[valign=c,width=0.19\textwidth]{figures/eq_6}
\includegraphics[valign=c,width=0.19\textwidth]{figures/eq_8} \\
\vspace*{0.35truecm}
\includegraphics[valign=c,width=0.19\textwidth]{figures/eq_10} 
\includegraphics[valign=c,width=0.19\textwidth]{figures/eq_12} 
\includegraphics[valign=c,width=0.19\textwidth]{figures/eq_14}
\includegraphics[valign=c,width=0.19\textwidth]{figures/eq_16}
\includegraphics[valign=c,width=0.19\textwidth]{figures/eq_18} \\
\vspace*{0.35truecm}
\includegraphics[valign=c,width=0.19\textwidth]{figures/eq_20} 
\includegraphics[valign=c,width=0.19\textwidth]{figures/eq_22} 
\includegraphics[valign=c,width=0.19\textwidth]{figures/eq_24}
\includegraphics[valign=c,width=0.19\textwidth]{figures/eq_26}
\includegraphics[valign=c,width=0.19\textwidth]{figures/eq_28} \\
\vspace*{0.35truecm}
\includegraphics[valign=c,width=0.19\textwidth]{figures/eq_30} 
\includegraphics[valign=c,width=0.19\textwidth]{figures/eq_32} 
\includegraphics[valign=c,width=0.19\textwidth]{figures/eq_34}
\includegraphics[valign=c,width=0.19\textwidth]{figures/eq_36}
\includegraphics[valign=c,width=0.19\textwidth]{figures/eq_38} \\
\vspace*{0.35truecm}
\includegraphics[valign=c,width=0.19\textwidth]{figures/eq_40} 
\includegraphics[valign=c,width=0.19\textwidth]{figures/eq_42}  \\
\caption{FEMA earthquake suite  (in g m/s-s).}
\label{eq_suite}
\end{center}
\end{figure}



\comnt{Megan, Add the Table here}

\begin{figure}
\includegraphics[width=\textwidth]{figures/table_place_holder.png}
\end{figure}


\subsection{Characterization of ground motion using SVD}
Once the ground motion suite is selected,  it needs to be processed for performing SVD according to \ref{PCA2}.  Since different ground motions have different sampling frequencies and record lengths, they were first interpolated to a common sampling frequency and record length. The common sampling frequency was chosen to be the 50Hz or a time step of 0.02s,  which corresponds to the largest sampling frequency among all the records.  The common time history length was chosen to be 90s, the longest record length in the suite.  For motions with duration less than 90s,  zero padding is used. This leads to $A_{4500 \times 44}$ in Equation \ref{PCA2} with $n$, number of time steps being equal to 4500 and $m$, number of earthquakes being equal to 44.  SVD was performed on matrix $A$, which resulted in a 44 column,  orthonormal basis matrix $U_{4500\times44}$.  First, the basis vectors are arranged in descending order of singular values,  and then the cumulative explained variance is plotted against the number of basis vectors in Figure \ref{exp_variance_cum}.  It can be observed that the first 40 basis vectors are responsible for explaining 99\% of variation in the ground motion data.  This result is reiterated in Figure \ref{exp_variance}, where the percentage of explained variance are plotted against the basis vector number.  Compared to the first 40 vectors,  the contribution of the the last 4 vectors are insignificant. Therefor,e only the first 40 vectors were chosen to be the basis vector for the ground motion suite leading to a $U_{4500 \times 40}$ orthonormal basis matrix.  Each of these 40 basis vectors are plotted in Figure \ref{eq_svd}.

\begin{figure}[h!]
\begin{center}
\subfigure[\label{exp_variance_cum} )]{\includegraphics[width=0.45\textwidth]{figures/exp_variance_cum}} 
\hspace*{0.2truecm}
\subfigure[\label{exp_variance} ]{\includegraphics[width=0.45\textwidth]{figures/exp_variance}} 
\caption{Explained variance}
\label{svd_efficiency}
\end{center}
\end{figure}

\begin{figure}
\begin{center}
\includegraphics[valign=c,width=0.19\textwidth]{figures/eq_basis_0} 
\includegraphics[valign=c,width=0.19\textwidth]{figures/eq_basis_1} 
\includegraphics[valign=c,width=0.19\textwidth]{figures/eq_basis_2}
\includegraphics[valign=c,width=0.19\textwidth]{figures/eq_basis_3}
\includegraphics[valign=c,width=0.19\textwidth]{figures/eq_basis_4} \\
\vspace*{0.35truecm}
\includegraphics[valign=c,width=0.19\textwidth]{figures/eq_basis_5} 
\includegraphics[valign=c,width=0.19\textwidth]{figures/eq_basis_6} 
\includegraphics[valign=c,width=0.19\textwidth]{figures/eq_basis_7}
\includegraphics[valign=c,width=0.19\textwidth]{figures/eq_basis_8}
\includegraphics[valign=c,width=0.19\textwidth]{figures/eq_basis_9} \\
\vspace*{0.35truecm}
\includegraphics[valign=c,width=0.19\textwidth]{figures/eq_basis_10} 
\includegraphics[valign=c,width=0.19\textwidth]{figures/eq_basis_11} 
\includegraphics[valign=c,width=0.19\textwidth]{figures/eq_basis_12}
\includegraphics[valign=c,width=0.19\textwidth]{figures/eq_basis_13}
\includegraphics[valign=c,width=0.19\textwidth]{figures/eq_basis_14} \\
\vspace*{0.35truecm}
\includegraphics[valign=c,width=0.19\textwidth]{figures/eq_basis_15} 
\includegraphics[valign=c,width=0.19\textwidth]{figures/eq_basis_16} 
\includegraphics[valign=c,width=0.19\textwidth]{figures/eq_basis_17}
\includegraphics[valign=c,width=0.19\textwidth]{figures/eq_basis_18}
\includegraphics[valign=c,width=0.19\textwidth]{figures/eq_basis_19} \\
\vspace*{0.35truecm}
\includegraphics[valign=c,width=0.19\textwidth]{figures/eq_basis_20} 
\includegraphics[valign=c,width=0.19\textwidth]{figures/eq_basis_21} 
\includegraphics[valign=c,width=0.19\textwidth]{figures/eq_basis_22}
\includegraphics[valign=c,width=0.19\textwidth]{figures/eq_basis_23}
\includegraphics[valign=c,width=0.19\textwidth]{figures/eq_basis_24} \\
\vspace*{0.35truecm}
\includegraphics[valign=c,width=0.19\textwidth]{figures/eq_basis_20} 
\includegraphics[valign=c,width=0.19\textwidth]{figures/eq_basis_21} 
\includegraphics[valign=c,width=0.19\textwidth]{figures/eq_basis_22}
\includegraphics[valign=c,width=0.19\textwidth]{figures/eq_basis_23}
\includegraphics[valign=c,width=0.19\textwidth]{figures/eq_basis_24} \\
\vspace*{0.35truecm}
\includegraphics[valign=c,width=0.19\textwidth]{figures/eq_basis_25} 
\includegraphics[valign=c,width=0.19\textwidth]{figures/eq_basis_26} 
\includegraphics[valign=c,width=0.19\textwidth]{figures/eq_basis_27}
\includegraphics[valign=c,width=0.19\textwidth]{figures/eq_basis_28}
\includegraphics[valign=c,width=0.19\textwidth]{figures/eq_basis_29} \\
\vspace*{0.35truecm}
\includegraphics[valign=c,width=0.19\textwidth]{figures/eq_basis_30} 
\includegraphics[valign=c,width=0.19\textwidth]{figures/eq_basis_31} 
\includegraphics[valign=c,width=0.19\textwidth]{figures/eq_basis_32}
\includegraphics[valign=c,width=0.19\textwidth]{figures/eq_basis_33}
\includegraphics[valign=c,width=0.19\textwidth]{figures/eq_basis_34} \\
\vspace*{0.35truecm}
\includegraphics[valign=c,width=0.19\textwidth]{figures/eq_basis_35} 
\includegraphics[valign=c,width=0.19\textwidth]{figures/eq_basis_36} 
\includegraphics[valign=c,width=0.19\textwidth]{figures/eq_basis_37}
\includegraphics[valign=c,width=0.19\textwidth]{figures/eq_basis_38}
\includegraphics[valign=c,width=0.19\textwidth]{figures/eq_basis_39} \\


\caption{FEMA earthquake suite basis (in g m/s-s).}
\label{eq_svd}
\end{center}
\end{figure}


\subsection{Training and testing the machine learning models}

To represent the FE models using machine learning models, one needs to train the ML models using a large set of input output pairs.  The output of the machine learning model is chosen to be the response of the building in terms of peak displacement and peak floor acceleration, which are typically used to predict structural and non-structural damages in buildings, respectively,  for risk assessment.  This resulted in a two dimensional output vector $Y$.  In order to train the machine learning model for a range of earthquakes and model parameters, the following steps were adopted \comnt{as outlined in Figure}.  

First, to produce training ground motions,  the FEMA P695 far-field ground motion suite was projected onto the $U$ basis,  which was obtained from SVD, as described in the previous section.  For each earthquake,  a set of 40 weights were obtained corresponding to each column vector of the $U$ basis, which form the columns of the weight matrix, $\Sigma _{40 \times 44}$ in Equation \ref{PCA2}.  Each column of the weight matrix ,$\Sigma$, was assumed to be a realization of an uniform random vector $\Teta_{1_{40 \times 1}}$. The bounds of $\Teta_1$ were chosen to be maximum and minimum values of each row of $\Sigma$.  This bound can be extended to capture a wider range of earthquake variation,  but for illustration of the framework this bound was chosen.  Now, one can produce new earthquakes by randomly generating values for $\Teta_1$ and multiplying it with $U$.  A few earthquakes corresponding to different realizations of $\Teta_1$ are shown in Figure \ref{eq_real}. 
\begin{figure}
\begin{center}
\includegraphics[valign=c,width=0.19\textwidth]{figures/eq_real_0} 
\includegraphics[valign=c,width=0.19\textwidth]{figures/eq_real_1} 
\includegraphics[valign=c,width=0.19\textwidth]{figures/eq_real_2}
\includegraphics[valign=c,width=0.19\textwidth]{figures/eq_real_3}
\includegraphics[valign=c,width=0.19\textwidth]{figures/eq_real_4} \\
\vspace*{0.35truecm}
\includegraphics[valign=c,width=0.19\textwidth]{figures/eq_real_5} 
\includegraphics[valign=c,width=0.19\textwidth]{figures/eq_real_6} 
\includegraphics[valign=c,width=0.19\textwidth]{figures/eq_real_7}
\includegraphics[valign=c,width=0.19\textwidth]{figures/eq_real_8}
\includegraphics[valign=c,width=0.19\textwidth]{figures/eq_real_9} \\

\caption{Earthquake realizations (in g m/s-s).}
\label{eq_real}
\end{center}
\end{figure}

Secondly,  to account for material variability,  the constitutive model parameters such as elastic modulus ($E$), yield stress ($F_y$),  and damping ratio ($\xi$) were chosen to be uniform random variables and mass of each story was assumed to be 1.0.  For each set of spring,  $E$ was chosen to be such that its natural period  varied between 0.75s-1.25s.  Mean of $F_y$ was chosen to be 5\% of the mean of the elastic modulus with bounds obtained by $\pm 20\%$ of the mean.  This choice of $F_y$ ensures that the response of the FE models reach the nonlinear regime for most of the realizations,  so that the machine learning model can be trained for non-linearity.  Mean of $\xi$ was chosen to be 0.05 with $\pm 20\%$ variation.  The ranges of the constitutive model parameters are shown in \ref{Table}.  This lead to a uniform random vector $\Teta_{2_{3 \times 1}}$ for the 1-DoF model, and $\Teta_{2 _{9 \times 1}}$ for the 3-DoF model.  Finally the input vector for the machine learning model $\Teta$ can be written as $\Teta=[Teta_1, Teta_2]^T$, which is a 43 dimensional vector for the 1-DoF model and the 49 dimensional vector for the 3-DoF model.  
 \begin{table}[h!]
\caption{Mean and support of the structural parameters,\comnt{placeholder}}
\label{hyperparameters}
\begin{center}
    \begin{tabular}{| c | c | c|}
    \hline
Parameter & Mean & Support\\
\hline \hline   
Elastic modulus($E$)  & 60 Pa  & [30,90]\\
\hline 
Yield stress ($F_y)$ & 12 Pa  & [10,15]\\
\hline 
Damping ratio ($\xi$) & 0.05  & [0.04,0.06]\\
\hline 
\end{tabular}
\end{center}
\end{table}


Once, the input random vector $\Teta$ and its PDF have been chosen,500,000 realizations were generated. The FE models were simulated for each of the realizations to obtain the two dimensional output vectors $Y$.  Force deformation plots for 10 arbitrarily chosen realizations are shown in Figure \ref{Force_Def_real}.  It can be noted that the chosen earthquakes and material parameters resulted in highly non-linear behavior and it was observed that about 99\% of all the realizations displayed non-linear behavior.  Next,in order to abstain from over-fitting,  of the 500,000 input-output data points, 90\% was used for training and 10\% was used for testing.  Now, the competing machine learning models were trained on the training input-output order pair and their performance was tested on the testing input-output order pair.  $R^2$ error  defined in Eq. \ref{r2}, was chosen as the performance metric:
\begin{equation}\label{r2}
R^2 (Y,\hat{Y})= 1-\frac{Variance(Y-(\hat{Y}))}{Variance({Y})}
\end{equation}
where the numerator is the error variance between the FE model output,  $Y$, and machine learning model output, $\hat{Y}$. 

It should be noted that choosing among the various competing machine learning models is a two step process.  It involves first choosing the best set of hyper parameters for a model type.. Once the best set of hyper-parameters are chosen then the best model is selected which produces the least $R^2$ error.  As mentioned earlier, a cross validation was done to chose the best hyper-parmeters for SVD,  DT and RF.   The hyper-parameters for DNN were chosen heuristically by varying the numbers of neurons and layers. The best values of hyper-parameters corresponding to each of the machine learning models mentioned in Section \ref{section4} are shown in Table \ref{}.   $R^2$ error for each of the machine learning model, corresponding to the best hyper parameters,  is shown in Figure \ref{test_train_1}-\ref{test_train_2}.  Figure \ref{test_train_1} (a) corresponds to the training error for the one-story building and \ref{test_train_1} (b) corresponds to the testing error for the one-story building. Similarly,  Figure \ref{test_train_2} (a) corresponds to the training error for the three-story building and \ref{test_train_2} (b) corresponds to the testing error for the three-story building.  It can be observed that the best performance is obtained by DNN in both training and testing, followed by RF, SVR and DT in both 1-DoF and 3-DoF case.  The merit of splitting the data can also be appreciated by checking the result for SVR in the 3-DoF case. It can be seen that SVR overfits the data as demonstrated by the low training error and high testing error.  Therefore,  the proposed model is a DNN with 10 layers and 500 neurons in each layer.  

Now, this model need to be validated before deploying. Even though the test set was not used for training the models, it was indirectly used for selection of hyper-parameters for SVR, RF and DT.  For DNN,  convergence of error on the testing set was used to stop the Forward and backward propagation loops. Therefore, in some sense there was leakage of information from the testing set to the training set. Moreover,  it might so happen that co-incidentally the model might perform well on one test set. Therefore, a thorough validation step is important before deploying the best performing machine learning model,  DNN in our case,  for use. 

%\begin{figure}[h!]
%\begin{center}
%\subfigure[\label{pdf_fy} ]{\includegraphics[width=0.32\textwidth]{figures/pdf_fy}} 
%\subfigure[\label{pdf_E} ]{\includegraphics[width=0.32\textwidth]{figures/pdf_E}} 
%\subfigure[\label{pdf_xi} ]{\includegraphics[width=0.32\textwidth]{figures/pdf_xi}} 
%\caption{PDFSs}
%\label{pdfs}
%\end{center}
%\end{figure}

%\begin{figure}
%\begin{center}
%\includegraphics[valign=c,width=0.19\textwidth]{figures/eq_real_0} 
%\includegraphics[valign=c,width=0.19\textwidth]{figures/eq_real_1} 
%\includegraphics[valign=c,width=0.19\textwidth]{figures/eq_real_2}
%\includegraphics[valign=c,width=0.19\textwidth]{figures/eq_real_3}
%\includegraphics[valign=c,width=0.19\textwidth]{figures/eq_real_4} \\
%\vspace*{0.35truecm}
%\includegraphics[valign=c,width=0.19\textwidth]{figures/eq_real_5} 
%\includegraphics[valign=c,width=0.19\textwidth]{figures/eq_real_6} 
%\includegraphics[valign=c,width=0.19\textwidth]{figures/eq_real_7}
%\includegraphics[valign=c,width=0.19\textwidth]{figures/eq_real_8}
%\includegraphics[valign=c,width=0.19\textwidth]{figures/eq_real_9} \\
%
%\caption{Earthquake realizations (in g m/s-s).}
%\label{eq_real}
%\end{center}
%\end{figure}

\begin{figure}
\begin{center}
\includegraphics[valign=c,width=0.19\textwidth]{figures/Force_Def_real_0} 
\includegraphics[valign=c,width=0.19\textwidth]{figures/Force_Def_real_1} 
\includegraphics[valign=c,width=0.19\textwidth]{figures/Force_Def_real_2}
\includegraphics[valign=c,width=0.19\textwidth]{figures/Force_Def_real_3}
\includegraphics[valign=c,width=0.19\textwidth]{figures/Force_Def_real_4} \\
\vspace*{0.35truecm}
\includegraphics[valign=c,width=0.19\textwidth]{figures/Force_Def_real_5} 
\includegraphics[valign=c,width=0.19\textwidth]{figures/Force_Def_real_6} 
\includegraphics[valign=c,width=0.19\textwidth]{figures/Force_Def_real_7}
\includegraphics[valign=c,width=0.19\textwidth]{figures/Force_Def_real_8}
\includegraphics[valign=c,width=0.19\textwidth]{figures/Force_Def_real_9} \\
\caption{Force-deformation plots.}
\label{Force_Def_real}
\end{center}
\end{figure}

 \begin{table}[h!]
\caption{Values of hyperparameters that gave the best result}
\label{hyperparameters}
\begin{center}
    \begin{tabular}{| c | c | c|}
    \hline
Machine Learning Model & Hyperparameters & Values\\
\hline \hline   
Decision trees (DT) & Depth, width  & [d=10, w=10\\
\hline 
Random forests (RF) & Depth, width  & [d=10, w=10\\
\hline 
Support vector regression (SVR) & Depth, width  & [d=10, w=10\\
\hline 
Deep neural networks (DNN) & Depth, width  & [d=10, w=10\\
\hline 
\end{tabular}
\end{center}
\end{table}

\comnt{Why dnn is better? Prashant}
\begin{figure}[h!]
\begin{center}
\subfigure[\label{1d_train} ]{\includegraphics[width=0.45\textwidth]{figures/1dof_train}} 
\hspace*{0.1truecm}
\subfigure[\label{1d_test} ]{\includegraphics[width=0.45\textwidth]{figures/1dof_test}} 
\caption{fff}
\label{test_train_1}
\end{center}
\end{figure}

\begin{figure}[h!]
\begin{center}
\subfigure[\label{3d_train}]{\includegraphics[width=0.45\textwidth]{figures/3dof_train}} 
\hspace*{0.1truecm}
\subfigure[\label{3d_test}]{\includegraphics[width=0.45\textwidth]{figures/3dof_test}} 
\caption{test }
\label{test_train_2}
\end{center}
\end{figure}


\subsection{Validation}

The selected DNN model was thoroughly validated. as explained in the following.  randomly generating 

\subsubsection{Using unseen generated earthquake and random parameters}
The validation effort starts with generating 50 realizations of $\Teta$ which results in 50 ground motions ($\Teta_1$) and 50 material parameters ($\Teta_2$).  To ensure that the generated earthquakes are different from the initial suite of 22 ground motion pairs,  various earthquake intensity measures are shown in Figure \ref{IMS}. In Figure \ref{IMS} (a), (b) and (c), we have compared the peak ground acceleration (PGA), Arias Intensity (IA) and first spectral moment, respectively,  of the generated earthquake motion with the original suite of earthquakes.  As it can be noted that these intensity measures are quite different from the original earthquakes and hence the generated earthquakes are considered as unseen earthquakes. 

The FE models were simulated for all the realization sets and the output $Y$ was obtained. The machine learning model was used to predict the output $Y$ using the input $\Teta$.  $R^2$ error was obtained for all 50 realizations. This entire process was repeated 100 times resulting in 100 $R^2$ errors. The median $R^2$ error was obtained to be 7\% for peak roof displacement and 4\% for peak floor acceleration for the 1-DoF case.  For the 3-DoF case, a median $R^2$ error of 8\% was observed for peak roof displacement and 6\% for peak floor acceleration.  These low values of $R^2$ errors were encouraging, given the machine learning model is predicting the response for unseen generated earthquakes.

\begin{figure}[h!]
\begin{center}
\subfigure[\label{pdf_fy} ]{\includegraphics[width=0.32\textwidth]{figures/PGA_gen}} 
\subfigure[\label{pdf_E} ]{\includegraphics[width=0.32\textwidth]{figures/Arias_gen}} 
\subfigure[\label{pdf_xi} ]{\includegraphics[width=0.32\textwidth]{figures/Moment_gen}} 
\caption{PDFSs}
\label{IMS}
\end{center}
\end{figure}


\subsection{Prediction for Loma prieta earthquake}

Next,  the DNN surrogate models of both the 1-DoF and 2-DoF systems were validated by predicting the response for the Loma Prieta earthquake recorded at the station Hollister - South and Pine.  This ground motion is not a part of the initial suite of 22 earthquakes, and therefore, successful prediction for this record will demonstrate the robustness of the surrogate model developed through the proposed framework.  The earthquake is first projected onto the $U$ basis and its weights were obtained according to Equation \ref{PCA3}. The reconstructed time history obtained by multiplying the weights with the $U$  basis is superimposed on the original ground motion as shown in Figure \ref{loma_prieta}. It can be seen that earthquake constructed using basis functions and weights can reproduce the actual record with considerable accuracy and can capture the overall features of the ground motion.  The intensity measures for both the original earthquake and reconstructed earthquake also showed a close match with 5\% 10\% and 8\% error for PGA,  Arias intensity and Spectral moment respectively. Since the earthquake is fixed,  $\Teta_1$ is deterministic.  5000 realizations of $\Teta_2$ were obtained to produce 5000 realization of the input vector $\Teta$.  The FEM model was simulated with the original earthquake and $\Teta_2$ as material parameters to obtain the output $Y$.  The surrogate model was fed in $\Teta$ to obtain the output $\hat{Y}$.  For the 1-DoF system, it was observed that the surrogate model could predict the peak displacement and the acceleration with a median error of 18\% and 9\%, respectively,  while that for the 3-DoF system, the median errors were 15\% (??) and 11\% (??), respectively.  Given that the ground motion was not considered a part of the initial suite of the 22 pairs,  these predictions are quite encouraging and based on this, the authors are fairly confident on the application of the proposed framework to predict response to far-field motions recorded at firm rock site.

\comnt{add the reconstructed motion on the same figure}
\begin{figure}
\begin{center}
\includegraphics[width=\textwidth]{figures/eq_basis_0} 
\end{center}
\label{loma_prieta}
\end{figure}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\section{Conclusion}\label{section4}

Performance based earthquake engineering framework is a benchmark decision making tool that is often limited by its high computational cost incurred by the probabilistic non-linear finite element analysis step in the framework while taking into account uncertainties in both earthquakes and constitutive parameters.  In this study,  the authors have made an attempt to develop a machine learning based surrogate model framework to accurately replicate finite element model response of a building for a given set of material parameters and far field ground motions recorded on firm rock site.  Challenge lies in training these surrogate models to predict for earthquakes because performance depends on the characteristic earthquake features used for training the ML models.  Traditional characterization techniques using intensity measures,  like Arias intensity,  PGA,  PGV, among others,  are relevant in giving information about a particular earthquake.  However,  due to the lack of an inverse relationship,  these measures cannot be used to generate ground motions that can be used in training, which is important to predict response for unseen earthquakes.  Moreover,  given a set of ground motion characteristics and model features,  different machine learning models perform differently. \comnt{Prashant}.  Therefore,  one needs to select a machine learning model that is specific to the input-output dataset.  To this end,  the authors propose a framework that a) characterizes ground motion in a fashion that can be used for training machine learning models and b) selects the best machine learning model that accurately replicates FE model output.  

The proposed framework  starts with selecting a representative suite of far field ground motions recorded on firm rock site.  Next,  an orthonormal basis is chosen that spans the space of the ground motion suite using singular value decomposition.  Assuming the weights of the basis vectors as random vectors and the constitutive parameters as random variables,  a large set of earthquakes and constitutive parameters are generated by random sampling.  The finite element model is simulated using these earthquakes and constitutive parameters.  Randomly generated weights and material parameters values along with the finite element model output serve as training data-set for the machine learning model.  Competing machine learning models are used such as decision trees,  random forests,  support vector regression and deep neural networks,  to map the input (weights of the basis vectors and constitutive model parameters) to the output (finite element model response).  The best model is then proposed based on some performance metric ($R^2$ error).  The proposed framework is illustrated on one-story and three-story buildings represented by spring-mass-damper systems, subjected to far field ground motions to predict peak roof displacement and peak floor acceleration.  Among the competing set of machine learning models, it was shown that deep neural networks can be used to accurately estimate non-linear response of the buildings subject to any unseen earthquake. This was validated by using the model to estimate building response for earthquakes and constitutive model parameters that were not a part of the training set,  for which the surrogate models could predict the response of the FE models with reasonable accuracy ($R^2$ error less than 20\%). Thus the proposed framework bolstered by validation results on unseen earthquakes provides a basis of optimism for the validity and applicability of the machine learning based surrogate model in predicting non-linear building response. 
 
\section{Future work}

Despite the good results this framework has certain limitations should be brought to the notice of the reader which would be addressed in future studies. These are summarized in the following.
\begin{itemize}
\item The authors are characterizing the far-field motions in this study for an initial demonstration of the proposed framework. These records are good representation of the characteristics of far-field motions on firm soil representing soil classes C and D and originating from strike slip and reverse thrust faults. In case one has to predict structural response for near-field motions or motions with long-period pulses (expected in soft soil), the initial ground motion suite needs to be expanded. In fact, the authors will extend the suite in a future study.
\item The illustrated framework uses SVD to span the space of the selected ground motion suite. This is a linear representation. Non-linear representation like radial basis functions , fourier basis, and GAM would be used in future studies. \comnt{Prashant}
\item Implementation of this framework would be done to more complicated, high fidelity finite element models. Computational judiciousness would be acomplished by using multi-fidelity deep neural network surrogate models where the surrogate for a low fidelity model would aid in directing the solution direction for the surrogate of a high fidelity model. This would help in achieving convergence for a low number of training data points. 
\end{itemize}


\bibliographystyle{model1-num-names}
\bibliography{SFEM,SoilProperties,allrefs,alex,Parida,Parida2,sysid,alexPaper,references}

\end{document}



==> figures/table_place_holder.tex <==
\input{Front Matter}
\linenumbers
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\section{Introduction}\label{section1}
\comnt{georgios, please read this paragraph and feel free to edit} The performance-based earthquake engineering (PBEE) framework, developed at \cite{Cornell:2000}, is a powerful tool that can express performance of civil infrastructures during future earthquakes in terms of many useful decision variables (DVs). This framework relies on four successive steps that include hazard analysis, finite element simulation, mapping EDPs to damage measures (DMs), and finally, decision-making by translating DMs to various DVs. Despite being an excellent framework for performance assessment,  its use is limited in complex civil infrastructures due to high computational costs, that arises from non-linear probabilistic FE simulation of the structure, considering uncertainties in future earthquakes that require incremental dynamic analysis  and constitutive material parameters \cite{Parida2020,ZAKERESTEGHAMATI2021112971}. To alleviate this computational burden, researchers often use surrogate models to compute EDPs.In its most common form, a surrogate model aims to derive a low computational cost mathematical function that directly maps the inputs to the finite element model to its output, by-passing the computationally expensive non-linear analysis.  Often, this mapping function is developed based on fundamental structural dynamic theory in conjunction with Newtonian mechanics. Such physics based approaches have found wide use in earthquake engineering practice due to underlying physical robustness and intuitiveness \cite{Guan_2021}. However, these methods often rely on many inherent simplistic assumptions, which can reduce the accuracy of response estimates.Contrast to physics-based approaches, data driven approaches develop the underlying mathematical mapping function based on training on a large set of input-output data.  Recently, machine learning models like logistic regression (LR),  decision trees (DT), random forest (RF), support vector regression (SVR), artificial neural networks among others are finding  traction in the civil engineering community as viable data-driven surrogate models tp predict EDPs for their ease of implementation and ability to capture high degree of non-linearity \cite{Padgett_ML_review}.  LR, RF and SVR based surrogate models have been used in \cite{ATAEI2015203} for fragility assessment of the deck unseating mode of failure for coastal bridges.  Mangalathu et al.\cite{Mang_RF} used RF to generate and update bridge specific fragility curves and ANN \cite{Mang_ANN} to derive multidimensional seismic fragility of single and two column bent, box-girder bridges.  Segura et al. \cite{Segura} used a polynomial response surface surrogate model to construct fragility surface  for efficient seismic assessment of gravity dams.  In Ref.\cite{Mang_boost} machine learning techniques with boosting algorithms is used for response prediction of reinforced concrete frame buildings.  In the aforementioned studies and many other similar works \cite{MOLLER2009432, kocamaz_binici_tuncay_2021,WU_2019, PEREZRAMIREZ2019603, AHMED2022103737, KIANI2019108},  it has been clearly demonstrated that that once the machine learning model is properly trained, it can replicate a non-linear finite element model output accurately.  It must be noted that a considerable computational effort is expended in the initial training of the machine models to replicate the non-linear behavior of the structure,  however, the value in these methods is drawn from the fact once trained subsequent estimation of non-linear prediction are computationally trivial.  Most studies in literature, however, train the data driven surrogate model for a particular suite of earthquakes.  changing the earthquake suite would necessitate retraining the surrogate model for a new set of earthquakes, which would lead to more computational expense.  A few studies like in Ref. \cite{Taflanidis} use krigging surrogate model in conjunction with stochastic ground motion models to predict non-linear structural response.  Uncertain parameters of the ground motion models and finite element models are used as inputs to the surrogate model to predict the structural response.  Even though this approach is an effective solution to the aforementioned \comnt{repeated training problem} but this framework is limited to only when the seismic risk assessment utilizes stochastic ground motion models which is rarely the case.  \comnt{Georgios and supratik, please help me here, this citation, why this limitation is bad}. Additionally, krigging is not a reliable method sinc.. \comnt{Prashant, lets write this part}. The authors believe that in order for the surrogate model to have any meaningful application, one needs to develop a method that uses characteristics from historical earthquake data to train the surrogate models, along with accounting for high degrees of non-linearity that may arise during an earthquake. 


This research paper aims to propose a machine learning based framework that would address the repeated training problem along with being highly accurate in capturing larger degrees of non-linearity.  In effect, this is akin to solving three simultaneous problems a) identifying an exhaustive set of input parameters that are a good representation of historic earthquake data, b) identifying a set of input parameters that capture sensitivity of finite element model to its parameters and c) identifying the best machine learning model that is not only able to capture the high degree of non-linearity but also high degree of variation in response that may arise due to variation in earthquake and material parameters.  To this end, this paper first discuses a systematic framework for  development of the surrogate model in Section \ref{section2}. Different challenges that might arise for training a surrogate model in the context of earthquake engineering are discussed along with proposing an ideal workflow needed for development of surrogate model is proposed. Next, in Section \ref{section3}, a singular value decomposition based earthquake characterization technique is put forward that aims to characterize earthquakes in a way meaningful for generating training data for the surrogate model.  This is followed by a brief discussion of various machine learning models relevant for the proposed framework in Section \ref{section4}.  In Section \ref{section5}, the framework is applied to train machine learning models to replicate non-linear response of a single story and three-story building finite element model to earthquake excitation.  The framework is validated using earthquakes and material parameters which have not been used in training. 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\section{Systematic Development of the Surrogate model}\label{section2}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
As mentioned earlier the research team proposed a machine learning based surrogate modeling framework that can be easily integrated into the PBEE framework for computationally inexpensive decision making. The objective of the machine learning model would be to predict the EDPs for a finite element (FE) model, for an earthquake and a set of constitutive parameter values. A systematic surrogate model framework to predict for the given earthquake and the model would as follows
\begin{itemize}
\item Generate numerous time-histories ``similar" to the given earthquake and material parameters ``similar'' to the actual model parameters of the dynamic system.
\item Simulate the FE model for these time histories and material parameters.
\item Train a ``suitable'' machine learning model with the results of the FEM model as output and the corresponding material parameters and time history features as input till a pre-selected error tolerance is achieved.
\item Prior to deployment, the surrogate model needs to be validated with unseen earthquakes and material parameters that have not not used in training. Only if it predicts EDPs with reasonable accuracy then the machine learning model can be deployed.  
\end{itemize}
This implies that any systematic development of a machine learning based surrogate model should include three stages a) selection of suitable features and generation of training data b)  selection of suitable machine learning model and c) validation of the model and deployment.  These stages in context of the current study are discussed in the following. 

\subsection{Selection of suitable features and generation of training data }\label{subsec1}
In order to train the model,one needs to create a training set of input variables that should include characteristics of earthquake time history and building model parameters which would affect the prediction of EDP. Once the set of input variables are decided, the finite element model is simulated for different realizations of the input variables and the corresponding EDPs are stored. The machine learning model is now trained using input-output data sets till satisfactory convergence is attained. Such a supervised learning method is quite common and has been carried out by \cite{MOLLER2009432, Mang_boost, ZAKERESTEGHAMATI2021112971}. When this supervised learning technique is extended to account for earthquake and building material uncertainty, two important problems need to be addressed. First, the input features chosen should be exhaustive for predicting EDPs with certain degree of accuracy and second, it should be possible to draw realizations of those input features and simulate the finite element model using them in order to obtain training output. Traditionally, earthquakes have been characterized using single valued parameters like peak frequency, corresponding Fourier amplitude, peak ground acceleration (PGA), peak ground velocity (PGV), pseudo-spectral acceleration, Arias intensity, spectral moment, among others. From a training point of view, such characterization parameters pose a problem, since it is impossible to generate earthquake time histories for different realizations of these parameters i.e.  no inverse relationship exists between these intensity measures and earthquake time histories. This implies that such parameters are not unique to an earthquake. Not only selection of features is important, but also the existence of an inverse relation so that enough training data can be generated is imperative. Therefore, instead of using traditional intensity measures of earthquake characterization the authors have proposed an alternative framework as illustrated in Section \ref{section3}.

\subsection{Selection of suitable machine learning model}\label{subsec2}
Machine learning models have been widely used in literature of earthquake engineering to tackle different problems, including surrogate modeling \cite{ATAEI2015203,MOLLER2009432, kocamaz_binici_tuncay_2021,WU_2019, PEREZRAMIREZ2019603, AHMED2022103737, KIANI2019108} . Depending on the available data,  objective and the complexity of the problem,  available computational expenditure and desired level of accuracy various machine learning models, like the simplistic multiple linear regression,  to the more complex artificial neural networks are available to choose from. Moreover,  even for a machine learning model of choice, one can would need to tune its hyperparameters that in turn affect their accuracy and efficiency. drastically\comnt{cite prashant paper} \cite{mangalthu}.  For example for a neural network, the number of neurons and layers can be adjsuted to affect its accuracy and efficiency \cite{Papadrakakis}. One can also think of the number of polynomial terms and their orders as hyperparmeters for a simple linear regression problem.  Selection of machine learning models and selection of hyper-parameters need to be systematically handled and have been discussed further in Section \ref{section4}.

\subsection{Validation of model and deployment}
\comnt{Prashant Sid}

\section{Framework for ground motion characterization}\label{section3}
Consider a set of $n$ earthquakes with $m$ times steps each. Following the theory of singular value decomposition (SVD) \cite{ }, one can represent the $n \times m$ matrix $A_{n \times m}$ of $n$ earthquakes as:
\begin{equation}\label{PCA1}
A_{n \times m}=U_{m \times n}^T S_{m \times q} V_{q \times m }
\end{equation}
where, $U_{n \times p}$ and $V_{q \times m }$ are orthonormal vectors and $S_{p \times q}$ is a diagonal matrix. $u_i$, columns of $U^T$ and $v_i$, columns of $V$, form bases for $n-dimensional$ and $m-dimensional$ column spaces respectively. Choosing $U^T$ as my $n$-dimensional basis, Equation \ref{PCA1} can be written as:
\begin{equation}\label{PCA2}
A_{n \times m}=U_{n \times p}^T \Sigma_{p \times m}
\end{equation}
where, $\Sigma$ is the matrix obtained by product of $S$ and $V$ matrices. Each column of $\Sigma$ consists of weights for the $u_i$s to produce the original earthquake suite $A$. For example, $i^{th}$ column of $A$, can be produced by multiplying the basis matrix $U^T$ with $i^{th}$ column of $\Sigma$. Therefore every earthquake can be characterized by a $p$-dimensional vector which can be fed to the machine learning model.  Now, to create a training set one can generate $p-dimensional$ random vectors an use it to produce corresponding time histories needed for training. Moreover, any new earthquake $P_{n \times 1}$ that the machine learning model would be used to predict EDPs, for can be projected onto the $U^T$ basis:
\begin{equation}
\sigma_{p \times 1} = U_{p \times n}P_{n \times 1}
\end{equation}
to obtain the $p$-dimensional weight vector $\sigma$ which is then fed to the machine-learning algorithm to make predictions.
\comnt{prashant and sid, need to add more to make it clearer to understand}

Please note that, the number of input variables increase with $p$. However, this can be taken are of by selecting a few components of the basis vector matrix $U^T$. This can be better understood by understanding the principal component (PC) interpretation of SVD.
\comnt{A flow shart should be added here illustrating the framework} 
 
\subsection{Principal component interpretation of SVD}
\comnt{prashant and sid}
when you write the equation, mention the number of principal components used as $l$.. something like
fdfdfddf
\begin{equation}\label{PCA3}
A_{n \times m}=U_{n \times l}^T \Sigma_{l \times m}
\end{equation}

 \begin{figure}[h!]
\begin{center}
\includegraphics[width=0.9\textwidth]{figures/pca}

\caption{PDFSs}
\label{pdfs}
\end{center}
\end{figure}


\subsection{Drawbacks/Limitations}
Please not that SVD is a linear transformation. There are other methods like Kernel PCA \comnt{prashant}, etc which project the data to a set of non-linear basis. These transformation and their impact on machine learning prediction would be a part of the research teams future endeavors. 

\section{Competing set of machine learning models}\label{section4}
\comnt{prashant and sid}
As mentioned earlier selection of a machine learning model,  and tuning its hyper-parameters is a complex problem affecting the surrogate models accuracy and efficiency. Therefore, a systematic approach needs to be carried out for selection of a suitable machine learning surrogate model.After going through extensive literature four algorithms were selected to be candidate surrogate models. A brief description of the models have been provided in the following.

\subsection{Decision trees(DT) and Random forest regression (RF)} Decision trees recursively partition the input space based on local regression models in the input space.  A greedy optimization algorithm with the objective of minimizing the loss between the prediction of the tree and the actual measurement is utilized to find the optimal partition of the input space. To overcome potential over-fitting with a single tree, RF creates a large number of trees with different branches and depths and averages the output as its prediction.  Such a method is called \textit{bagging} where the average of a number of models result in an unbiased model. Number of DTs in the RF model and the maximum depth of each DT are two important tuning parameters that affect efficiency and accuracy of the prediction. 

\subsection{Support vector regression(SVR)} SVR use non-linear kernel function to map data into high-dimensional feature space. In this feature space, it is expected that the data attains more ``favorable" features which is then captured by a simple linear regression.  SVR is robust to over-fitting. and also provides flexibility by kernel selection.  Tuning parameters are type of kernel function, regularization parameter and  the allowed error tolerance ($\epsilon$) for the linear regression in high dimensional feature space.     

\subsection{Deep neural networks (DNN)} A deep network typically consists of an input layer, an output layer and a stack of hidden layers connecting the input layer to the output layer.  The hidden layers project the inputs into spaces of different dimensions via various linear and non-linear projections and produce the model output.  One hidden layer feeds into another via a linear transformation and within a hidden layer, the output of the previous layer is undergone a non-parametric non-linear transformation. The process is repeated for all hidden layers up until the output layers.  This stage is called forward propagation. Weights of the linear transformations can be obtained by minimizing the mean square error, loss between the model predicted output and the actual data.  This is done by back propagating the loss gradient via chain rule.  In this study, the rectified linear unit (ReLU) is used as non-linear transformation within a hidden layer \cite{}. This is because ReLU activation functions are more efficient and are generally shown to be best for deep neural networks because of fewer vanishing gradients problems when it is back-propagated through the hidden layers \cite{}. \comnt{Prashant} as compared to other activation functions like sigmoid.  

For DT, RF,  and SVR a cross validation approach is used to find optimal set of hyperparameters that best predict the data. In the case of DNN the optimal values of number of neurons and layers were decided heuristically by running several different number of neurons and layer combinations as suggested in \cite{Papadrakakis}.  Of the tuned machine learning models the winner is selected on the basis of some performance metric

\section{Results and Discussion}\label{section5}

\subsection{1Dof and 3Dof FEM models}
To illustrate the proposed framework,  one-story and three-story buildings are considered,  which are modeled as spring-mass-damper system in OpenSEES \cite{opensees}.  Chopra \cite{chopra2000dynamics} indicates that in most cases,  the first mode,  or the first few modes of a multi-degree of freedom stick model of the structure can provide useful approximation of the total response of the building,  and therefore, considered here. The springs are assumed to be uniaxial bilinear steel material with kinematic hardening with no isotropic hardening, and are modeled using the Steel01 \cite{} material in OpenSEES.  Elastic material element with specified damping stiffness was used in parallel with the non-linear spring to capture the damping behavior of the material.   For the one-story building, only one set of parallel springs are used, while for the three story building, three set of parallel springs are used in series. The objective of the problem is to accurately predict the response of these FE models for an earthquake,  using machine learning  given a set of values for spring constitutive model parameters.%The yield strength of the spring are so selected such that the response of the FE models reach the nonlinear regime,  so that we have enough data to capture the nonlinearity in training the surrogate model.  


\subsection{Choice of initial suite of ground motion}
As discussed earlier, the ground motion selection is one of the most important factors in training and developing accurate surrogate models, as the suite needs to be a good representation of an unseen excitation.  In this study, a set of 22 pair of ground motions representing magnitudes of range 6.5-7.6 recorded on firm soil (rock or stiff, $V_s$ > 180 m/s) were selected from the \cite{} \comnt{FEMA P695} far-field suite. The list of the selected ground motions and their characteristics are presented in \ref{table1}\comnt{Table 1}. All these ground motions are recorded at sites located greater than or equal to 10 km from fault rupture (strike slip and reverse thrust), referred to as “Far-Field” motions. To ensure broad representation of different recorded earthquakes, this set contain far-field records selected from most large-magnitude events in the PEER NGA database \cite{} \comnt{PEER, 2006}. The inherent differences in event magnitude, distance to source, source type and site conditions of these ground motions considers the record-to-record variability that is essential to capture the ground motion uncertainties. More information on the record selection criteria can be found in \cite{} \comnt{FEMA P695}. Figure \ref{eq_suite} shows the acceleration time histories of one component from each pair of ground motion in the earthquake suite. 
\begin{figure}
\begin{center}
\includegraphics[valign=c,width=0.19\textwidth]{figures/eq_0} 
\includegraphics[valign=c,width=0.19\textwidth]{figures/eq_2} 
\includegraphics[valign=c,width=0.19\textwidth]{figures/eq_4}
\includegraphics[valign=c,width=0.19\textwidth]{figures/eq_6}
\includegraphics[valign=c,width=0.19\textwidth]{figures/eq_8} \\
\vspace*{0.35truecm}
\includegraphics[valign=c,width=0.19\textwidth]{figures/eq_10} 
\includegraphics[valign=c,width=0.19\textwidth]{figures/eq_12} 
\includegraphics[valign=c,width=0.19\textwidth]{figures/eq_14}
\includegraphics[valign=c,width=0.19\textwidth]{figures/eq_16}
\includegraphics[valign=c,width=0.19\textwidth]{figures/eq_18} \\
\vspace*{0.35truecm}
\includegraphics[valign=c,width=0.19\textwidth]{figures/eq_20} 
\includegraphics[valign=c,width=0.19\textwidth]{figures/eq_22} 
\includegraphics[valign=c,width=0.19\textwidth]{figures/eq_24}
\includegraphics[valign=c,width=0.19\textwidth]{figures/eq_26}
\includegraphics[valign=c,width=0.19\textwidth]{figures/eq_28} \\
\vspace*{0.35truecm}
\includegraphics[valign=c,width=0.19\textwidth]{figures/eq_30} 
\includegraphics[valign=c,width=0.19\textwidth]{figures/eq_32} 
\includegraphics[valign=c,width=0.19\textwidth]{figures/eq_34}
\includegraphics[valign=c,width=0.19\textwidth]{figures/eq_36}
\includegraphics[valign=c,width=0.19\textwidth]{figures/eq_38} \\
\vspace*{0.35truecm}
\includegraphics[valign=c,width=0.19\textwidth]{figures/eq_40} 
\includegraphics[valign=c,width=0.19\textwidth]{figures/eq_42}  \\
\caption{FEMA earthquake suite  (in g m/s-s).}
\label{eq_suite}
\end{center}
\end{figure}



\comnt{Megan, Add the Table here}

\begin{figure}
\includegraphics[width=\textwidth]{figures/table_place_holder.png}
\end{figure}


\subsection{Characterization of ground motion using SVD}
Once the ground motion suite is selected,  it needs to be processed for performing SVD according to \ref{PCA2}.  Since different ground motions have different sampling frequencies and record lengths, they were first interpolated to a common sampling frequency and record length. The common sampling frequency was chosen to be the 50Hz or a time step of 0.02s,  which corresponds to the largest sampling frequency among all the records.  The common time history length was chosen to be 90s, the longest record length in the suite.  For motions with duration less than 90s,  zero padding is used. This leads to $A_{4500 \times 44}$ in Equation \ref{PCA2} with $n$, number of time steps being equal to 4500 and $m$, number of earthquakes being equal to 44.  SVD was performed on matrix $A$, which resulted in a 44 column,  orthonormal basis matrix $U_{4500\times44}$.  First, the basis vectors are arranged in descending order of singular values,  and then the cumulative explained variance is plotted against the number of basis vectors in Figure \ref{exp_variance_cum}.  It can be observed that the first 40 basis vectors are responsible for explaining 99\% of variation in the ground motion data.  This result is reiterated in Figure \ref{exp_variance}, where the percentage of explained variance are plotted against the basis vector number.  Compared to the first 40 vectors,  the contribution of the the last 4 vectors are insignificant. Therefor,e only the first 40 vectors were chosen to be the basis vector for the ground motion suite leading to a $U_{4500 \times 40}$ orthonormal basis matrix.  Each of these 40 basis vectors are plotted in Figure \ref{eq_svd}.

\begin{figure}[h!]
\begin{center}
\subfigure[\label{exp_variance_cum} )]{\includegraphics[width=0.45\textwidth]{figures/exp_variance_cum}} 
\hspace*{0.2truecm}
\subfigure[\label{exp_variance} ]{\includegraphics[width=0.45\textwidth]{figures/exp_variance}} 
\caption{Explained variance}
\label{svd_efficiency}
\end{center}
\end{figure}

\begin{figure}
\begin{center}
\includegraphics[valign=c,width=0.19\textwidth]{figures/eq_basis_0} 
\includegraphics[valign=c,width=0.19\textwidth]{figures/eq_basis_1} 
\includegraphics[valign=c,width=0.19\textwidth]{figures/eq_basis_2}
\includegraphics[valign=c,width=0.19\textwidth]{figures/eq_basis_3}
\includegraphics[valign=c,width=0.19\textwidth]{figures/eq_basis_4} \\
\vspace*{0.35truecm}
\includegraphics[valign=c,width=0.19\textwidth]{figures/eq_basis_5} 
\includegraphics[valign=c,width=0.19\textwidth]{figures/eq_basis_6} 
\includegraphics[valign=c,width=0.19\textwidth]{figures/eq_basis_7}
\includegraphics[valign=c,width=0.19\textwidth]{figures/eq_basis_8}
\includegraphics[valign=c,width=0.19\textwidth]{figures/eq_basis_9} \\
\vspace*{0.35truecm}
\includegraphics[valign=c,width=0.19\textwidth]{figures/eq_basis_10} 
\includegraphics[valign=c,width=0.19\textwidth]{figures/eq_basis_11} 
\includegraphics[valign=c,width=0.19\textwidth]{figures/eq_basis_12}
\includegraphics[valign=c,width=0.19\textwidth]{figures/eq_basis_13}
\includegraphics[valign=c,width=0.19\textwidth]{figures/eq_basis_14} \\
\vspace*{0.35truecm}
\includegraphics[valign=c,width=0.19\textwidth]{figures/eq_basis_15} 
\includegraphics[valign=c,width=0.19\textwidth]{figures/eq_basis_16} 
\includegraphics[valign=c,width=0.19\textwidth]{figures/eq_basis_17}
\includegraphics[valign=c,width=0.19\textwidth]{figures/eq_basis_18}
\includegraphics[valign=c,width=0.19\textwidth]{figures/eq_basis_19} \\
\vspace*{0.35truecm}
\includegraphics[valign=c,width=0.19\textwidth]{figures/eq_basis_20} 
\includegraphics[valign=c,width=0.19\textwidth]{figures/eq_basis_21} 
\includegraphics[valign=c,width=0.19\textwidth]{figures/eq_basis_22}
\includegraphics[valign=c,width=0.19\textwidth]{figures/eq_basis_23}
\includegraphics[valign=c,width=0.19\textwidth]{figures/eq_basis_24} \\
\vspace*{0.35truecm}
\includegraphics[valign=c,width=0.19\textwidth]{figures/eq_basis_20} 
\includegraphics[valign=c,width=0.19\textwidth]{figures/eq_basis_21} 
\includegraphics[valign=c,width=0.19\textwidth]{figures/eq_basis_22}
\includegraphics[valign=c,width=0.19\textwidth]{figures/eq_basis_23}
\includegraphics[valign=c,width=0.19\textwidth]{figures/eq_basis_24} \\
\vspace*{0.35truecm}
\includegraphics[valign=c,width=0.19\textwidth]{figures/eq_basis_25} 
\includegraphics[valign=c,width=0.19\textwidth]{figures/eq_basis_26} 
\includegraphics[valign=c,width=0.19\textwidth]{figures/eq_basis_27}
\includegraphics[valign=c,width=0.19\textwidth]{figures/eq_basis_28}
\includegraphics[valign=c,width=0.19\textwidth]{figures/eq_basis_29} \\
\vspace*{0.35truecm}
\includegraphics[valign=c,width=0.19\textwidth]{figures/eq_basis_30} 
\includegraphics[valign=c,width=0.19\textwidth]{figures/eq_basis_31} 
\includegraphics[valign=c,width=0.19\textwidth]{figures/eq_basis_32}
\includegraphics[valign=c,width=0.19\textwidth]{figures/eq_basis_33}
\includegraphics[valign=c,width=0.19\textwidth]{figures/eq_basis_34} \\
\vspace*{0.35truecm}
\includegraphics[valign=c,width=0.19\textwidth]{figures/eq_basis_35} 
\includegraphics[valign=c,width=0.19\textwidth]{figures/eq_basis_36} 
\includegraphics[valign=c,width=0.19\textwidth]{figures/eq_basis_37}
\includegraphics[valign=c,width=0.19\textwidth]{figures/eq_basis_38}
\includegraphics[valign=c,width=0.19\textwidth]{figures/eq_basis_39} \\


\caption{FEMA earthquake suite basis (in g m/s-s).}
\label{eq_svd}
\end{center}
\end{figure}


\subsection{Training and testing the machine learning models}

To represent the FE models using machine learning models, one needs to train the ML models using a large set of input output pairs.  The output of the machine learning model is chosen to be the response of the building in terms of peak displacement and peak floor acceleration, which are typically used to predict structural and non-structural damages in buildings, respectively,  for risk assessment.  This resulted in a two dimensional output vector $Y$.  In order to train the machine learning model for a range of earthquakes and model parameters, the following steps were adopted \comnt{as outlined in Figure}.  

First, to produce training ground motions,  the FEMA P695 far-field ground motion suite was projected onto the $U$ basis,  which was obtained from SVD, as described in the previous section.  For each earthquake,  a set of 40 weights were obtained corresponding to each column vector of the $U$ basis, which form the columns of the weight matrix, $\Sigma _{40 \times 44}$ in Equation \ref{PCA2}.  Each column of the weight matrix ,$\Sigma$, was assumed to be a realization of an uniform random vector $\Teta_{1_{40 \times 1}}$. The bounds of $\Teta_1$ were chosen to be maximum and minimum values of each row of $\Sigma$.  This bound can be extended to capture a wider range of earthquake variation,  but for illustration of the framework this bound was chosen.  Now, one can produce new earthquakes by randomly generating values for $\Teta_1$ and multiplying it with $U$.  A few earthquakes corresponding to different realizations of $\Teta_1$ are shown in Figure \ref{eq_real}. 
\begin{figure}
\begin{center}
\includegraphics[valign=c,width=0.19\textwidth]{figures/eq_real_0} 
\includegraphics[valign=c,width=0.19\textwidth]{figures/eq_real_1} 
\includegraphics[valign=c,width=0.19\textwidth]{figures/eq_real_2}
\includegraphics[valign=c,width=0.19\textwidth]{figures/eq_real_3}
\includegraphics[valign=c,width=0.19\textwidth]{figures/eq_real_4} \\
\vspace*{0.35truecm}
\includegraphics[valign=c,width=0.19\textwidth]{figures/eq_real_5} 
\includegraphics[valign=c,width=0.19\textwidth]{figures/eq_real_6} 
\includegraphics[valign=c,width=0.19\textwidth]{figures/eq_real_7}
\includegraphics[valign=c,width=0.19\textwidth]{figures/eq_real_8}
\includegraphics[valign=c,width=0.19\textwidth]{figures/eq_real_9} \\

\caption{Earthquake realizations (in g m/s-s).}
\label{eq_real}
\end{center}
\end{figure}

Secondly,  to account for material variability,  the constitutive model parameters such as elastic modulus ($E$), yield stress ($F_y$),  and damping ratio ($\xi$) were chosen to be uniform random variables and mass of each story was assumed to be 1.0.  For each set of spring,  $E$ was chosen to be such that its natural period  varied between 0.75s-1.25s.  Mean of $F_y$ was chosen to be 5\% of the mean of the elastic modulus with bounds obtained by $\pm 20\%$ of the mean.  This choice of $F_y$ ensures that the response of the FE models reach the nonlinear regime for most of the realizations,  so that the machine learning model can be trained for non-linearity.  Mean of $\xi$ was chosen to be 0.05 with $\pm 20\%$ variation.  The ranges of the constitutive model parameters are shown in \ref{Table}.  This lead to a uniform random vector $\Teta_{2_{3 \times 1}}$ for the 1-DoF model, and $\Teta_{2 _{9 \times 1}}$ for the 3-DoF model.  Finally the input vector for the machine learning model $\Teta$ can be written as $\Teta=[Teta_1, Teta_2]^T$, which is a 43 dimensional vector for the 1-DoF model and the 49 dimensional vector for the 3-DoF model.  
 \begin{table}[h!]
\caption{Mean and support of the structural parameters,\comnt{placeholder}}
\label{hyperparameters}
\begin{center}
    \begin{tabular}{| c | c | c|}
    \hline
Parameter & Mean & Support\\
\hline \hline   
Elastic modulus($E$)  & 60 Pa  & [30,90]\\
\hline 
Yield stress ($F_y)$ & 12 Pa  & [10,15]\\
\hline 
Damping ratio ($\xi$) & 0.05  & [0.04,0.06]\\
\hline 
\end{tabular}
\end{center}
\end{table}


Once, the input random vector $\Teta$ and its PDF have been chosen,500,000 realizations were generated. The FE models were simulated for each of the realizations to obtain the two dimensional output vectors $Y$.  Force deformation plots for 10 arbitrarily chosen realizations are shown in Figure \ref{Force_Def_real}.  It can be noted that the chosen earthquakes and material parameters resulted in highly non-linear behavior and it was observed that about 99\% of all the realizations displayed non-linear behavior.  Next,in order to abstain from over-fitting,  of the 500,000 input-output data points, 90\% was used for training and 10\% was used for testing.  Now, the competing machine learning models were trained on the training input-output order pair and their performance was tested on the testing input-output order pair.  $R^2$ error  defined in Eq. \ref{r2}, was chosen as the performance metric:
\begin{equation}\label{r2}
R^2 (Y,\hat{Y})= 1-\frac{Variance(Y-(\hat{Y}))}{Variance({Y})}
\end{equation}
where the numerator is the error variance between the FE model output,  $Y$, and machine learning model output, $\hat{Y}$. 

It should be noted that choosing among the various competing machine learning models is a two step process.  It involves first choosing the best set of hyper parameters for a model type.. Once the best set of hyper-parameters are chosen then the best model is selected which produces the least $R^2$ error.  As mentioned earlier, a cross validation was done to chose the best hyper-parmeters for SVD,  DT and RF.   The hyper-parameters for DNN were chosen heuristically by varying the numbers of neurons and layers. The best values of hyper-parameters corresponding to each of the machine learning models mentioned in Section \ref{section4} are shown in Table \ref{}.   $R^2$ error for each of the machine learning model, corresponding to the best hyper parameters,  is shown in Figure \ref{test_train_1}-\ref{test_train_2}.  Figure \ref{test_train_1} (a) corresponds to the training error for the one-story building and \ref{test_train_1} (b) corresponds to the testing error for the one-story building. Similarly,  Figure \ref{test_train_2} (a) corresponds to the training error for the three-story building and \ref{test_train_2} (b) corresponds to the testing error for the three-story building.  It can be observed that the best performance is obtained by DNN in both training and testing, followed by RF, SVR and DT in both 1-DoF and 3-DoF case.  The merit of splitting the data can also be appreciated by checking the result for SVR in the 3-DoF case. It can be seen that SVR overfits the data as demonstrated by the low training error and high testing error.  Therefore,  the proposed model is a DNN with 10 layers and 500 neurons in each layer.  

Now, this model need to be validated before deploying. Even though the test set was not used for training the models, it was indirectly used for selection of hyper-parameters for SVR, RF and DT.  For DNN,  convergence of error on the testing set was used to stop the Forward and backward propagation loops. Therefore, in some sense there was leakage of information from the testing set to the training set. Moreover,  it might so happen that co-incidentally the model might perform well on one test set. Therefore, a thorough validation step is important before deploying the best performing machine learning model,  DNN in our case,  for use. 

%\begin{figure}[h!]
%\begin{center}
%\subfigure[\label{pdf_fy} ]{\includegraphics[width=0.32\textwidth]{figures/pdf_fy}} 
%\subfigure[\label{pdf_E} ]{\includegraphics[width=0.32\textwidth]{figures/pdf_E}} 
%\subfigure[\label{pdf_xi} ]{\includegraphics[width=0.32\textwidth]{figures/pdf_xi}} 
%\caption{PDFSs}
%\label{pdfs}
%\end{center}
%\end{figure}

%\begin{figure}
%\begin{center}
%\includegraphics[valign=c,width=0.19\textwidth]{figures/eq_real_0} 
%\includegraphics[valign=c,width=0.19\textwidth]{figures/eq_real_1} 
%\includegraphics[valign=c,width=0.19\textwidth]{figures/eq_real_2}
%\includegraphics[valign=c,width=0.19\textwidth]{figures/eq_real_3}
%\includegraphics[valign=c,width=0.19\textwidth]{figures/eq_real_4} \\
%\vspace*{0.35truecm}
%\includegraphics[valign=c,width=0.19\textwidth]{figures/eq_real_5} 
%\includegraphics[valign=c,width=0.19\textwidth]{figures/eq_real_6} 
%\includegraphics[valign=c,width=0.19\textwidth]{figures/eq_real_7}
%\includegraphics[valign=c,width=0.19\textwidth]{figures/eq_real_8}
%\includegraphics[valign=c,width=0.19\textwidth]{figures/eq_real_9} \\
%
%\caption{Earthquake realizations (in g m/s-s).}
%\label{eq_real}
%\end{center}
%\end{figure}

\begin{figure}
\begin{center}
\includegraphics[valign=c,width=0.19\textwidth]{figures/Force_Def_real_0} 
\includegraphics[valign=c,width=0.19\textwidth]{figures/Force_Def_real_1} 
\includegraphics[valign=c,width=0.19\textwidth]{figures/Force_Def_real_2}
\includegraphics[valign=c,width=0.19\textwidth]{figures/Force_Def_real_3}
\includegraphics[valign=c,width=0.19\textwidth]{figures/Force_Def_real_4} \\
\vspace*{0.35truecm}
\includegraphics[valign=c,width=0.19\textwidth]{figures/Force_Def_real_5} 
\includegraphics[valign=c,width=0.19\textwidth]{figures/Force_Def_real_6} 
\includegraphics[valign=c,width=0.19\textwidth]{figures/Force_Def_real_7}
\includegraphics[valign=c,width=0.19\textwidth]{figures/Force_Def_real_8}
\includegraphics[valign=c,width=0.19\textwidth]{figures/Force_Def_real_9} \\
\caption{Force-deformation plots.}
\label{Force_Def_real}
\end{center}
\end{figure}

 \begin{table}[h!]
\caption{Values of hyperparameters that gave the best result}
\label{hyperparameters}
\begin{center}
    \begin{tabular}{| c | c | c|}
    \hline
Machine Learning Model & Hyperparameters & Values\\
\hline \hline   
Decision trees (DT) & Depth, width  & [d=10, w=10\\
\hline 
Random forests (RF) & Depth, width  & [d=10, w=10\\
\hline 
Support vector regression (SVR) & Depth, width  & [d=10, w=10\\
\hline 
Deep neural networks (DNN) & Depth, width  & [d=10, w=10\\
\hline 
\end{tabular}
\end{center}
\end{table}

\comnt{Why dnn is better? Prashant}
\begin{figure}[h!]
\begin{center}
\subfigure[\label{1d_train} ]{\includegraphics[width=0.45\textwidth]{figures/1dof_train}} 
\hspace*{0.1truecm}
\subfigure[\label{1d_test} ]{\includegraphics[width=0.45\textwidth]{figures/1dof_test}} 
\caption{fff}
\label{test_train_1}
\end{center}
\end{figure}

\begin{figure}[h!]
\begin{center}
\subfigure[\label{3d_train}]{\includegraphics[width=0.45\textwidth]{figures/3dof_train}} 
\hspace*{0.1truecm}
\subfigure[\label{3d_test}]{\includegraphics[width=0.45\textwidth]{figures/3dof_test}} 
\caption{test }
\label{test_train_2}
\end{center}
\end{figure}


\subsection{Validation}

The selected DNN model was thoroughly validated. as explained in the following.  randomly generating 

\subsubsection{Using unseen generated earthquake and random parameters}
The validation effort starts with generating 50 realizations of $\Teta$ which results in 50 ground motions ($\Teta_1$) and 50 material parameters ($\Teta_2$).  To ensure that the generated earthquakes are different from the initial suite of 22 ground motion pairs,  various earthquake intensity measures are shown in Figure \ref{IMS}. In Figure \ref{IMS} (a), (b) and (c), we have compared the peak ground acceleration (PGA), Arias Intensity (IA) and first spectral moment, respectively,  of the generated earthquake motion with the original suite of earthquakes.  As it can be noted that these intensity measures are quite different from the original earthquakes and hence the generated earthquakes are considered as unseen earthquakes. 

The FE models were simulated for all the realization sets and the output $Y$ was obtained. The machine learning model was used to predict the output $Y$ using the input $\Teta$.  $R^2$ error was obtained for all 50 realizations. This entire process was repeated 100 times resulting in 100 $R^2$ errors. The median $R^2$ error was obtained to be 7\% for peak roof displacement and 4\% for peak floor acceleration for the 1-DoF case.  For the 3-DoF case, a median $R^2$ error of 8\% was observed for peak roof displacement and 6\% for peak floor acceleration.  These low values of $R^2$ errors were encouraging, given the machine learning model is predicting the response for unseen generated earthquakes.

\begin{figure}[h!]
\begin{center}
\subfigure[\label{pdf_fy} ]{\includegraphics[width=0.32\textwidth]{figures/PGA_gen}} 
\subfigure[\label{pdf_E} ]{\includegraphics[width=0.32\textwidth]{figures/Arias_gen}} 
\subfigure[\label{pdf_xi} ]{\includegraphics[width=0.32\textwidth]{figures/Moment_gen}} 
\caption{PDFSs}
\label{IMS}
\end{center}
\end{figure}


\subsection{Prediction for Loma prieta earthquake}

Next,  the DNN surrogate models of both the 1-DoF and 2-DoF systems were validated by predicting the response for the Loma Prieta earthquake recorded at the station Hollister - South and Pine.  This ground motion is not a part of the initial suite of 22 earthquakes, and therefore, successful prediction for this record will demonstrate the robustness of the surrogate model developed through the proposed framework.  The earthquake is first projected onto the $U$ basis and its weights were obtained according to Equation \ref{PCA3}. The reconstructed time history obtained by multiplying the weights with the $U$  basis is superimposed on the original ground motion as shown in Figure \ref{loma_prieta}. It can be seen that earthquake constructed using basis functions and weights can reproduce the actual record with considerable accuracy and can capture the overall features of the ground motion.  The intensity measures for both the original earthquake and reconstructed earthquake also showed a close match with 5\% 10\% and 8\% error for PGA,  Arias intensity and Spectral moment respectively. Since the earthquake is fixed,  $\Teta_1$ is deterministic.  5000 realizations of $\Teta_2$ were obtained to produce 5000 realization of the input vector $\Teta$.  The FEM model was simulated with the original earthquake and $\Teta_2$ as material parameters to obtain the output $Y$.  The surrogate model was fed in $\Teta$ to obtain the output $\hat{Y}$.  For the 1-DoF system, it was observed that the surrogate model could predict the peak displacement and the acceleration with a median error of 18\% and 9\%, respectively,  while that for the 3-DoF system, the median errors were 15\% (??) and 11\% (??), respectively.  Given that the ground motion was not considered a part of the initial suite of the 22 pairs,  these predictions are quite encouraging and based on this, the authors are fairly confident on the application of the proposed framework to predict response to far-field motions recorded at firm rock site.

\comnt{add the reconstructed motion on the same figure}
\begin{figure}
\begin{center}
\includegraphics[width=\textwidth]{figures/eq_basis_0} 
\end{center}
\label{loma_prieta}
\end{figure}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\section{Conclusion}\label{section4}

Performance based earthquake engineering framework is a benchmark decision making tool that is often limited by its high computational cost incurred by the probabilistic non-linear finite element analysis step in the framework while taking into account uncertainties in both earthquakes and constitutive parameters.  In this study,  the authors have made an attempt to develop a machine learning based surrogate model framework to accurately replicate finite element model response of a building for a given set of material parameters and far field ground motions recorded on firm rock site.  Challenge lies in training these surrogate models to predict for earthquakes because performance depends on the characteristic earthquake features used for training the ML models.  Traditional characterization techniques using intensity measures,  like Arias intensity,  PGA,  PGV, among others,  are relevant in giving information about a particular earthquake.  However,  due to the lack of an inverse relationship,  these measures cannot be used to generate ground motions that can be used in training, which is important to predict response for unseen earthquakes.  Moreover,  given a set of ground motion characteristics and model features,  different machine learning models perform differently. \comnt{Prashant}.  Therefore,  one needs to select a machine learning model that is specific to the input-output dataset.  To this end,  the authors propose a framework that a) characterizes ground motion in a fashion that can be used for training machine learning models and b) selects the best machine learning model that accurately replicates FE model output.  

The proposed framework  starts with selecting a representative suite of far field ground motions recorded on firm rock site.  Next,  an orthonormal basis is chosen that spans the space of the ground motion suite using singular value decomposition.  Assuming the weights of the basis vectors as random vectors and the constitutive parameters as random variables,  a large set of earthquakes and constitutive parameters are generated by random sampling.  The finite element model is simulated using these earthquakes and constitutive parameters.  Randomly generated weights and material parameters values along with the finite element model output serve as training data-set for the machine learning model.  Competing machine learning models are used such as decision trees,  random forests,  support vector regression and deep neural networks,  to map the input (weights of the basis vectors and constitutive model parameters) to the output (finite element model response).  The best model is then proposed based on some performance metric ($R^2$ error).  The proposed framework is illustrated on one-story and three-story buildings represented by spring-mass-damper systems, subjected to far field ground motions to predict peak roof displacement and peak floor acceleration.  Among the competing set of machine learning models, it was shown that deep neural networks can be used to accurately estimate non-linear response of the buildings subject to any unseen earthquake. This was validated by using the model to estimate building response for earthquakes and constitutive model parameters that were not a part of the training set,  for which the surrogate models could predict the response of the FE models with reasonable accuracy ($R^2$ error less than 20\%). Thus the proposed framework bolstered by validation results on unseen earthquakes provides a basis of optimism for the validity and applicability of the machine learning based surrogate model in predicting non-linear building response. 
 
\section{Future work}

Despite the good results this framework has certain limitations should be brought to the notice of the reader which would be addressed in future studies. These are summarized in the following.
\begin{itemize}
\item The authors are characterizing the far-field motions in this study for an initial demonstration of the proposed framework. These records are good representation of the characteristics of far-field motions on firm soil representing soil classes C and D and originating from strike slip and reverse thrust faults. In case one has to predict structural response for near-field motions or motions with long-period pulses (expected in soft soil), the initial ground motion suite needs to be expanded. In fact, the authors will extend the suite in a future study.
\item The illustrated framework uses SVD to span the space of the selected ground motion suite. This is a linear representation. Non-linear representation like radial basis functions , fourier basis, and GAM would be used in future studies. \comnt{Prashant}
\item Implementation of this framework would be done to more complicated, high fidelity finite element models. Computational judiciousness would be acomplished by using multi-fidelity deep neural network surrogate models where the surrogate for a low fidelity model would aid in directing the solution direction for the surrogate of a high fidelity model. This would help in achieving convergence for a low number of training data points. 
\end{itemize}


\bibliographystyle{model1-num-names}
\bibliography{SFEM,SoilProperties,allrefs,alex,Parida,Parida2,sysid,alexPaper,references}

\end{document}


